Learned Two-Plane Perspective Prior based Image Resampling for Efficient Object Detection

Real-time efficient perception is critical for autonomous navigation and city scale sensing. Orthogonal to architectural improvements, streaming perception approaches have exploited adaptive sampling improving real-time detection performance. In this work, we propose a learnable geometry-guided prior that incorporates rough geometry of the 3D scene (a ground plane and a plane above) to resample images for efficient object detection. This significantly improves small and far-away object detection performance while also being more efficient both in terms of latency and memory. For autonomous navigation, using the same detector and scale, our approach improves detection rate by +4.1 $AP_{S}$ or +39% and in real-time performance by +5.3 $sAP_{S}$ or +63% for small objects over state-of-the-art (SOTA). For fixed traffic cameras, our approach detects small objects at image scales other methods cannot. At the same scale, our approach improves detection of small objects by 195% (+12.5 $AP_{S}$) over naive-downsampling and 63% (+4.2 $AP_{S}$) over SOTA.

==> busedge.tex <==

\redX{-- Drive-by sensing, transit systems can act as sustainable sensors for the city for monitoring road conditions~\cite{mohannericell}, public service infrastructure~\cite{Ye-2021-128891}, HD map updates~\cite{Bu-2022-133236} etc. -- Edge execution necessary because single bus with 7 cameras at 5 fps captures a million frames everyday.  -- US has half a million school buses alone~\cite{schoolbuses}. Too much data for cloud.  -- Edge devices are resource constrained, along with latency, memory also becomes important. -- Jetson devices have 8 to 16 GB RAM shared between GPU and CPU cores, and for ML on multiple streams, spatial downsampling is necessary. --- In the considered scenario, VP is fixed, so we can cache saliency S. -- Our results on Busedge Accessibility shows we consume xx memory which yy times less than baseline, while real-time performance improvement of \green{aa} sAP.}
